Pattern-based design applied to cultural heritage knowledge graphs

Ontology Design Patterns (ODPs) have become an established and recognised practice for guaranteeing good quality ontology engineering. There are several ODP repositories where ODPs are shared as well as ontology design methodologies recommending their reuse. Performing rigorous testing is recommended as well for supporting ontology maintenance and validating the resulting resource against its motivating requirements. Nevertheless, it is less than straightforward to find guidelines on how to apply such methodologies for developing domain-specific knowledge graphs. ArCo is the knowledge graph of Italian Cultural Heritage and has been developed by using eXtreme Design (XD), an ODP- and test-driven methodology. During its development, XD has been adapted to the need of the CH domain e.g. gathering requirements from an open, diverse community of consumers, a new ODP has been defined and many have been specialised to address specific CH requirements. This paper presents ArCo and describes how to apply XD to the development and validation of a CH knowledge graph, also detailing the (intellectual) process implemented for matching the encountered modelling problems to ODPs. Relevant contributions also include a novel web tool for supporting unit-testing of knowledge graphs, a rigorous evaluation of ArCo, and a discussion of methodological lessons learned during ArCo development.

==> sections/cqs.tex <==
\begin{table*}[htp]
\begin{center}
	\caption{Representative competency questions answered by ArCo ontology network.}
	\label{tab:arco-cq}
	\begin{tabular}{p{0.5cm}p{15cm}}
		\hline
		{ \bf ID } & { \bf Competency question }\\\hline 
		{ \bf } & { \bf ArCo module }\\\hline 
		CQ\theCQscounter{} & Is a cultural property tangible or intangible?\\\hline
		CQ\incrementCQscounter & Is a cultural property movable or immovable?\\\hline
		CQ\incrementCQscounter & What are the cultural properties of a given type?\\\hline
		CQ\incrementCQscounter & What are the components of a complex cultural property?\\\hline
		CQ\incrementCQscounter & What is/are the residual(s) of a cultural property?\\\hline
		CQ\incrementCQscounter & Which is the catalogue record describing a cultural property?\\\hline
		{ \bf } & { \bf Catalogue module }\\\hline
		CQ\incrementCQscounter & Which is the level of detail of the catalogue record?\\\hline
		CQ\incrementCQscounter & When was a catalogue record created or updated? \\\hline
		CQ\incrementCQscounter & Which are all the versions of a catalogue record? \\\hline
		CQ\incrementCQscounter & Which is the (immediate) previous catalogue record version of a catalogue record version? And which is the (immediate) next one? \\\hline
		CQ\incrementCQscounter & Who, and playing which role, was responsible for creating, editing and updating a catalogue record? \\\hline
		CQ\incrementCQscounter & What is, and for what reason, the level of privacy of a catalogue record? \\\hline
		{ \bf } & { \bf Location module }\\\hline
		CQ\incrementCQscounter & What are all the places where a cultural property has been located? Which are their types?\\\hline
		CQ\incrementCQscounter & When a cultural property has been located in a place?\\\hline
		CQ\incrementCQscounter & Which are the geographical coordinates of a cultural property? \\\hline
		CQ\incrementCQscounter & Which are the cadastral data associated to the cultural property location? \\\hline
		{ \bf } & { \bf Denotative description module}\\\hline
		CQ\incrementCQscounter & What is the conservation status of a cultural property?\\\hline
		CQ\incrementCQscounter & What is the technical status of a cultural property?\\\hline
		CQ\incrementCQscounter & What are the measurements of a cultural property? \\\hline
		CQ\incrementCQscounter & What are the elements, e.g. inscriptions, affixed on a cultural property? \\\hline
		{ \bf } & { \bf Context description module}\\\hline
		CQ\incrementCQscounter & What are the authors and/or cultural scopes attributed to a cultural property?\\\hline
		CQ\incrementCQscounter & When a cultural property has been created? \\\hline
		CQ\incrementCQscounter & Which is the subject represented on a cultural property? \\\hline
		CQ\incrementCQscounter & Which are the current and/or previous owners of a cultural property? \\\hline
		CQ\incrementCQscounter & Who commissioned a cultural property? \\\hline
		CQ\incrementCQscounter & Which are the bibliography and documentation related to a cultural property? \\\hline
		CQ\incrementCQscounter & Which interventions and surveys have been carried out on a cultural property? \\\hline
		CQ\incrementCQscounter & Which collection a cultural property is member of? \\\hline
		{ \bf } & { \bf Cultural event module}\\\hline
		CQ\theCQscounter{} & In which cultural events and exhibitions a cultural property has been involved?\\\hline
		CQ\incrementCQscounter & Which cultural properties have been involved in a cultural event?\\\hline
		CQ\incrementCQscounter & What are the events of a recurrent event series?\\\hline
		CQ\incrementCQscounter & Which is the time period elapsing between two events of a recurrent event series?\\\hline
		CQ\incrementCQscounter & What are the unifying criteria shared by all the events in a recurrent event series?\\\hline
	\end{tabular}
	\end{center}
\end{table*}
